EvalCrafter: Benchmarking and Evaluating Large Video Generation Models

The vision and language generative models have been overgrown in recent years. For video generation, various open-sourced models and public-available services have been developed to generate high-quality videos. However, these methods often use a few metrics, e.g., FVD or IS, to evaluate the performance. We argue that it is hard to judge the large conditional generative models from the simple metrics since these models are often trained on very large datasets with multi-aspect abilities. Thus, we propose a novel framework and pipeline for exhaustively evaluating the performance of the generated videos. Our approach involves generating a diverse and comprehensive list of 700 prompts for text-to-video generation, which is based on an analysis of real-world user data and generated with the assistance of a large language model. Then, we evaluate the state-of-the-art video generative models on our carefully designed benchmark, in terms of visual qualities, content qualities, motion qualities, and text-video alignment with 17 well-selected objective metrics. To obtain the final leaderboard of the models, we further fit a series of coefficients to align the objective metrics to the users' opinions. Based on the proposed human alignment method, our final score shows a higher correlation than simply averaging the metrics, showing the effectiveness of the proposed evaluation method.

==> figs/bench.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/ours_new.pdf}
    \caption{We consider over 4 main meta types to evaluate the performance of the types of the generated video, where each type contains several prompts with fine-grained attribute labels. For each prompt, we also consider the motion and the style of the video, yet more diverse prompts. \xiaodong{todo: replace the figure, can remove}}
    \label{fig:bench}
\end{figure}


==> figs/correlation.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/correlation.png}
    \caption{Results' correlation with \textit{SL}. We calculate the correlation between \textit{SL} with our EvalCrafter results (on \textit{OVQ,  TVA,  MQ, TC,}  and \textit{EvalCrafter-SL}.) as well as the directly average Average-SL. It should be a Table for comparison.}
    \label{fig:correlation}
\end{figure}


==> figs/model_comparison.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/Overall_Comparison.png}
    \vspace{-2em}
    \caption{Skill-aware comparison }
    \label{fig:comparison}
\end{figure*}

==> figs/word_freq.tex <==
% Use figure* for multi-column figure
% Use figure* for multi-column figure
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/wordcloud2.png}
    \caption{A placeholder for the real-word prompt distribution.}
    \label{fig:word_freq}
\end{figure}


==> figs/xtype.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/output.png}
    \caption{The evaluation of the model in different types}
    \label{fig:xtype}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/stability.tex <==
\begin{table}[h]
\centering
\vspace{-1em}
\resizebox{\columnwidth}{!}{%

\begin{tabular}{@{}lccccc@{}}
\toprule
% Model & Video Quality & TV-Align & Motion & Temporal & Total \\ \midrule
{} & Visual & Text-Video & Motion & Temporal \\ 
{} & Quality & Alignment & Quality & Consistency \\ \midrule

ModelScope & +0.01 & +0.63 & $\pm$0.00 & -0.04 \\
VideoCrafter1 & +0.06 & +0.05 & $\pm$0.00 & +0.01\\
ZeroScope & -0.05 & +0.35 & $\pm$0.00 & -0.13 \\ \bottomrule
\end{tabular}
}
\vspace{-1em}
\caption{Results' changes after noised. }
\vspace{-1.3em}
\end{table}
